DSOL: A Fast Direct Sparse Odometry Scheme

In this paper, we describe Direct Sparse Odometry Lite (DSOL), an improved version of Direct Sparse Odometry (DSO). We propose several algorithmic and implementation enhancements which speed up computation by a significant factor (on average 5x) even on resource constrained platforms. The increase in speed allows us to process images at higher frame rates, which in turn provides better results on rapid motions. Our open-source implementation is available at https://github.com/versatran01/dsol.

==> img/result/tta_dsol.tex <==
\begin{figure*}
\begin{subfigure}[b]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/data/dsol_tta_carwelding_002_3d.png}
    \caption{carwelding}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/data/dsol_tta_gascola_003_3d.png}
    \caption{gascola}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/data/dsol_tta_office_001_3d.png}
    \caption{office}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/data/dsol_tta_office2_005_3d.png}
    \caption{office2}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/data/dsol_tta_oldtown_000_3d.png}
    \caption{oldtown}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/data/dsol_tta_hospital_000_3d.png}
    \caption{hospital}
\end{subfigure}
\caption{Qualitative results of \dsol~on selected sequences from TartanAir~\cite{Wang2020TartanAirAD}.
Green lines are groundtruth trajectories, red lines are estimated trajectories.
Better viewed in color and zoomed in.
\chao{May be move this to first page as ian suggested? 2x3}
}
\label{fig:result/tta_dsol}
\vspace{-8px}
\end{figure*}
